Tartar: A Lightweight Raw-Waveform Keyword Spotting Model

Keyword spotting (KWS) is a common always-on, machine-learning workload for edge devices. End-to-end models that classify raw waveforms avoid expensive preprocessing, previously shown to be a bottleneck, but lightweight deployment still requires jointly tuning accuracy against both MAC and non-MAC costs. We present Tartar, a raw-waveform KWS model that is 'tunable' with a carefully selected set of architectural parameters, enabling trading accuracy against hardware cost. When evaluating Tartar, we find that non-MAC layers significantly impact the hardware cost. We introduce a lossless compression technique and its hardware implementation that significantly reduces the non-MAC cost. Tartar achieves 95.93% accuracy on the Google Speech Commands Dataset v2 with an implementation of only 4,028 LUTs, 8 DSPs, and 16 BRAMs. Compared against the closest competing KWS model, Tartar uses 7x fewer LUTs and 10x fewer DSPs, while remaining competitive in accuracy.

==> tikz/pipeline_mic.tex <==
% Shared microphone icon — https://tex.stackexchange.com/questions/396518/microphone-in-tikz
\providecommand{\pipelinemic}{%
  \tikz{
    \begin{scope}
      \clip (-.3em,-.4ex) rectangle (1.3em,1.5ex);
      \fill[black, rounded corners=1.5ex] (-.3em,-.4ex) rectangle (1.3em,5.5ex);
    \end{scope}
    \fill[white, rounded corners=1.3ex] (-.1em,0) rectangle (1.1em,5.1ex);
    \fill[black, rounded corners=1.1ex] (0,.2ex) rectangle (1em,5ex);
    \foreach \pos in {2.5ex, 2.9ex, 3.3ex, 3.7ex}
      \fill[white, rounded corners=.1ex] (.35em,\pos) rectangle +(.8em,.25ex);
    \fill[black] (.4em,-.4ex) rectangle (.6em,-1.5ex);
    \fill[black] (0,-1.5ex) rectangle (1em,-2ex);
  }%
}

